On the Effectiveness of Weight-Encoded Neural Implicit 3D Shapes

A neural implicit outputs a number indicating whether the given query point in space is inside, outside, or on a surface. Many prior works have focused on _latent-encoded_ neural implicits, where a latent vector encoding of a specific shape is also fed as input. While affording latent-space interpolation, this comes at the cost of reconstruction accuracy for any _single_ shape. Training a specific network for each 3D shape, a _weight-encoded_ neural implicit may forgo the latent vector and focus reconstruction accuracy on the details of a single shape. While previously considered as an intermediary representation for 3D scanning tasks or as a toy-problem leading up to latent-encoding tasks, weight-encoded neural implicits have not yet been taken seriously as a 3D shape representation. In this paper, we establish that weight-encoded neural implicits meet the criteria of a first-class 3D shape representation. We introduce a suite of technical contributions to improve reconstruction accuracy, convergence, and robustness when learning the signed distance field induced by a polygonal mesh -- the _de facto_ standard representation. Viewed as a lossy compression, our conversion outperforms standard techniques from geometry processing. Compared to previous latent- and weight-encoded neural implicits we demonstrate superior robustness, scalability, and performance.

==> acks.tex <==
derek and towaki 
Mike roberts (apple guy) for suggestion back prop for normals.
twitter haha


==> fig/accuracySlider.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.5\linewidth]{fig/fig_accuracySlider.pdf}
  \vspace{-10pt}
  \caption{\label{accuracySlider}As network complexity increases, the \repName reconstruction quality increases while rendering speed decreases. Depending on the application varying levels of accuracy can be achieved.}
  \vspace{-6pt}
  \label{fig:accuracySlider}
\end{figure}

==> fig/architecture.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{fig/fig_architecture.pdf}
  \vspace{-15pt}
  \caption{\label{fig:architecture}\netName\ network architecture. Given point samples of an object's SDF (left), we train a feed-forward neural network (middle) to predict the signed distances (right) of each input point.}
  \vspace{-10pt}
\end{figure}

==> fig/awesomeSDF.tex <==
\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{10pt}%
\begin{wrapfigure}[12]{r}{0.45\linewidth}
    \vspace{-0.2mm} % fine tuning layout
      \centering
      \includegraphics[width=1.0\linewidth]{fig/awesomeSDF.png}
      %\caption
      %\vspace{-20pt} % fine tuning layout
      %\caption{Complex implicit functions can be constructed through
      %combinations of primitives and "playing" with the math. Typically
      %requiring numerous tricks and design iterations to generate desired
      %shaped.}% https://www.shadertoy.com/view/ld3Gz2}
      %\vspace{-10pt} % fine tuning layout
\end{wrapfigure}


==> fig/importanceSampling.tex <==
\begin{figure}[t!]
%\vspace{-10pt} % careful: this extra vspace is here because of [b!]
  \begin{center}
%     \begin{subfigure}{.32\linewidth}
 %     \centering
      \includegraphics[width=.32\columnwidth]{fig/GingeruniformSampling.png}
  %  \end{subfigure}
    %\begin{subfigure}{0.32\linewidth}
     % \centering
      \includegraphics[width=.32\columnwidth]{fig/GingerweightedSampling.png}
    %\end{subfigure}
    %\begin{subfigure}{0.32\linewidth}
    %  \centering
      \includegraphics[width=.32\columnwidth]{fig/GingerimportanceSampling.png}
    %\end{subfigure}
    \end{center}
    \vspace{-7pt}
  \caption{Our importance sampling (right) draws a subset of points from a uniform sample set (left) according to their distance to the surface (middle).}
  \vspace{-10pt}
  \label{fig:importanceOverview}
\end{figure}

==> fig/importanceSamplingMotivation.tex <==
\begin{wrapfigure}[]{r}{0.5\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/fig_importanceCompare.pdf}
  \vspace{-20pt}
  \caption{\label{fig:importanceCompare}Visualizing sample density of samples when drawing $10^4$ points using: (left to right) vertex sampling with $\mathcal{N}(p,0.1)$ offsets~\cite{chen2018implicit_decoder}, surface sampling with $\mathcal{N}(p,0.01)$~\cite{Park_deepsdf}, and our importance sampling approach with $w=e^{-30|SDF(p)|}$.  We color samples according to their density estimated with Gaussian kernel density, normalized by the most dense region from vertex sampling.}
\end{wrapfigure}

==> fig/non-manifold.tex <==
\begin{wrapfigure}[]{r}{\linewidth}
  \includegraphics[width=\linewidth]{fig/fig_swat-wn-distance}
    %\vspace{-15pt}
\caption{Our conversion process supports non-watertight meshes with open
  boundaries, self intersections, and non-manifold edges.}
  %\vspace{-15pt}
\label{fig:nonmanifold}
\end{wrapfigure}


==> fig/sdf.tex <==
\begin{wrapfigure}[8]{r}{0.25\linewidth}
\centering
  \vspace{-15pt}
  \hspace{-30pt}
  \includegraphics[width=1.2\linewidth]{fig/bunnysdf.pdf}
\end{wrapfigure}

==> fig/sdfOperations.tex <==
\begin{wrapfigure}[]{r}{0.5\linewidth}
  \centering
  \vspace{-12 pt}
  \includegraphics[width=\linewidth]{fig/fig_sdfOperations.pdf}
  \vspace{-12 pt}
  \caption{\repName s admit many trivial interactive manipulations, the models predicted distance's can be modified through boolean operations similar to any implicit field. See accompanying video for animation.}
  \label{fig:sdfops}
  \vspace{-12 pt}
\end{wrapfigure}

==> fig/sharpEdge.tex <==
\begin{wrapfigure}[]{r}{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/fig_sharpEdge.pdf}
    \caption{Our \repName\ format encodes sharp edges with a high degree of accuracy.}
    \vspace{-10pt} % fine tuning layout
    \label{fig:sharpEdge}
\end{wrapfigure}

==> fig/windingnumber.tex <==
\begin{figure}[]
  \centering
     \begin{subfigure}{.243\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig/closeddistance.png}
    \end{subfigure}
    \begin{subfigure}{0.243\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig/closedwinding.png}
    \end{subfigure}
    \begin{subfigure}{0.243\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig/openDistance.png}
    \end{subfigure}
    \begin{subfigure}{0.243\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig/openWinding.png}
    \end{subfigure}
    \vspace{-10pt}
  \caption{Generalized winding number provides a smooth gradient from "inside" to "outside" in the presence of open boundaries.}
  \vspace{-15pt}
\end{figure}

==> related.tex <==
\section{Related Work} \label{related}

\subsection{3d Representations}
There have been a number of successful 3D representation for learning based
geometric tasks. 

Grid based approaches, specifically voxels, are a common approach for
generative\cite{Maturana2015VoxNet} and discrimitive\cite{choy20163d} tasks. Due
to memory limitations these early approaches are typically restricted to
resolutions of $32^3$ voxel grids until more recent work applying convolutions
to voxels grids \cite{marrnet} or nested tree structure approaches (octrees)
\cite{Wang-2018-AOCNN}. These improvements improve the overall resolution of
voxel grids, but are still limited to $256^3$ resolutions and can require to
overly complex implementations to achieve.

A point cloud is an unordered list of points created by sampling a surface in
memory, or scanning an object in reality. Point clouds are a natural fit for
deep learning due to their simplicity, efficiency, and lightweight memory
impact. PointNet \cite{qi2016pointnet} introduced deep learning on point clouds
applying a fully connected layer to each point independently followed by a
global pooling operation to extract shape level features. (\textbf{any point
referencing others?}). An obvious limitation of these approaches coming from
their ambiguous topology resulting in complex algorithms to produce a surface on
output \cite{Bernardini:1999:BAS:614276.614442}. 

Recently, there have been a number of works focusing on using polygon meshes
themselves as the representation for deep learning. These approaches of the
obvious benefit of producing a closed mesh on output. Mesh based machine
learning has been achieved by applying convolutions on the graph created between
vertices and edges of the mesh
\cite{Bronsteinaf5}. Prone to self intersecting
meshes, simple fixed topology, object class template, or cannot generate closed
surfaces.  \cite{wang2018pixel2mesh} 


\subsection{Learning implicit fields}
Recently there have been a number of works using implicit fields as a
representation for geometric learning tasks such as classification, single image
reconstruction and generative modelling. 

\cite{Park_deepsdf} 
\cite{Mescheder_Occupancy_Networks}
\cite{chen2018implicit_decoder}
\cite{Littwin_2019}

\cite{atzmon2019sal}
\cite{deprelle2019learning}
\cite{smirnov2019deep}
\cite{jiang2019sdfdiff}

\subsection{Rendering Learnt Implicit Fields}

\cite{niemeyer2019differentiable}
\cite{jiang2019sdfdiff}
\cite{liu2019dist}

